Twits, Toxic Tweets, and Tribal Tendencies: Trends in Politically Polarized Posts on Twitter

Social media platforms are often blamed for exacerbating political polarization and worsening public dialogue. Many claim that hyperpartisan users post pernicious content, slanted to their political views, inciting contentious and toxic conversations. However, what factors are actually associated with increased online toxicity and negative interactions? In this work, we explore the role that partisanship and affective polarization play in contributing to toxicity both on an individual user level and a topic level on Twitter/X. To do this, we train and open-source a DeBERTa-based toxicity detector with a contrastive objective that outperforms the Google Jigsaw Perspective Toxicity detector on the Civil Comments test dataset. Then, after collecting 89.6 million tweets from 43,151 Twitter/X users, we determine how several account-level characteristics, including partisanship along the US left-right political spectrum and account age, predict how often users post toxic content. Fitting a Generalized Additive Model to our data, we find that the diversity of views and the toxicity of the other accounts with which that user engages has a more marked effect on their own toxicity. Namely, toxic comments are correlated with users who engage with a wider array of political views. Performing topic analysis on the toxic content posted by these accounts using the large language model MPNet and a version of the DP-Means clustering algorithm, we find similar behavior across 5,288 individual topics, with users becoming more toxic as they engage with a wider diversity of politically charged topics.

==> communities.tex <==
\section{Communities}
Having our outlined our techniques for determining the political orientation and toxicity levels of different subreddits, we now turn to understanding how misinformation interacts in subreddits of different political leanings and toxicity levels. 



\subsection{Exponential Random Graph Models}
In order to model some of the interactions between online toxicity, misinformation levels, and polarization levels, we utilize exponential random graphs. Exponential Random Graph Modeling (ERGM), is a network models are a form of random graphs that predict connections between different nodes in a given network~\cite{hunter2008ergm}. ERGM models assume that connections are determined by a random variable $p^*$ that is dependent on input variables.  As in Chen \textit{et al.}~\cite{chen2022misleading} and Peng \textit{et al.}~\cite{peng2016follower}. We utilize this modelling as it does it does not assume that its data input is independent; given that we want to model the interactions of polarization, toxicity, and misinformation levels, this relaxed restriction is key. Furthermore, ERGMs can be efficiently computed with random Markov Chain Monte Carlo processes allowing us to model the large amounts of interactions between subreddits and between user in our dataset~\cite{van2019introduction,hunter2008ergm}.

==> dead.tex <==
\subsection{Twitter Dataset}
 For our Twitter dataset, we collected the Tweets of a set of users that tweeted conspiracy theory, misinformation, or authentic news websites from their profile. Utilizing our set of conspiracy theory, misinformation, and authentic news websites and the Python \texttt{Tweepy} we collected the usernames of profiles that tweeted these domains throughout December 2021, totaling 181K different Twitter users. For each of these users, utilizing the \texttt{Tweepy} API we then collected each of their most recent 3240 tweets. Altogether this totaled 446,439,819 different tweets.
 
 In addition, to this core dataset, in order to understand the larger Twitter ecosystem and the relative toxicity and the amounts of misinformation on the platform, we also we utilize the Twitter Streaming API. The Twitter Streaming API gives real-time access to 1\% of public tweets. We continuously collected these tweets between July 10 and and December 21, 2020. We utilize this dataset to understand the characteristics of users within the US-focused and highly politically engaged English-language Twitter ecosystem as a whole. 
 
 
 
 \begin{figure}
    \centering

\begin{tikzpicture}[very thick]
    % Right square
    \node[fill=gray!20,draw=red, minimum size=2cm, inner sep=0pt] (as) {$1.08\%$};
    \node[draw=black,minimum size=2cm, inner sep=0pt, above=-\pgflinewidth of as] (abh) {$0.94\%$};
    \node[draw=black,minimum size=2cm, inner sep=0pt, right=-\pgflinewidth of as] (abv) {$0.87\%$};
    \node[fill=gray!20,draw=blue, minimum size=2cm, inner sep=0pt,  above right=-\pgflinewidth and -\pgflinewidth of as]  {$1.24\%$};
    
    % Side labels
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=1.0cm] at (as.west) {Conservative};
    \node[anchor=north,] at (as.south) {Liberal};
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=0.6cm] at (abh.west) {Liberal};
    \node[anchor=north] at (abv.south) {Conservative};
    
    
    % Square label
    \node[xshift=1cm, below=0.7cm of as] {Target};
    
    \node[yshift=1.50cm,xshift=-0.75cm,rotate=90,left=0.5cm of as] {Author};

\end{tikzpicture}
  \caption{Percentage of interactions that are toxic/uncivil in misinformation submissions}
    \label{fig:my_label}
    
\end{figure}    

\begin{figure}
    \centering

\begin{tikzpicture}[very thick]
    % Right square
    \node[fill=gray!20,draw=red, minimum size=2cm, inner sep=0pt] (as) {$0.78\%$};
    \node[draw=black,minimum size=2cm, inner sep=0pt, above=-\pgflinewidth of as] (abh) {$0.83\%$};
    \node[draw=black,minimum size=2cm, inner sep=0pt, right=-\pgflinewidth of as] (abv) {$0.82\%$};
    \node[fill=gray!20,draw=blue, minimum size=2cm, inner sep=0pt,  above right=-\pgflinewidth and -\pgflinewidth of as]  {$0.76\%$};
    
    % Side labels
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=1.0cm] at (as.west) {Conservative};
    \node[anchor=north,] at (as.south) {Liberal};
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=0.6cm] at (abh.west) {Liberal};
    \node[anchor=north] at (abv.south) {Conservative};
    
    
    % Square label
    \node[xshift=1cm, below=0.7cm of as] {Target};
    
    \node[yshift=1.50cm,xshift=-0.75cm,rotate=90,left=0.5cm of as] {Author};

\end{tikzpicture}
  \caption{Percentage of interactions that are toxic/uncivil in mainstream submission}
    \label{fig:my_label}
    
\end{figure}   

\begin{table}[b]
\centering
\begin{tabular}{ll}
\toprule
   \multicolumn{2}{c}{\large Toxic Interactions}          \\
   \toprule
      \midrule
      Intercept              & -8.545 ***  &-8.530*** \\               
      \midrule
      User Polarization               & -0.292 & -0.464 \\
      \midrule
      User Polarization Differences    & -2.040*** &-0.782 *** \\
    \midrule
       User Toxicity &   10.557*** &  12.396***\\
      \midrule
       Reciprocity &   3.0863*** &  4.568***\\
      \midrule
\bottomrule
& $\ast p<0.05; ** p<0.01; *** p<0.001$ \\
\end{tabular}
\caption{Caption\label{time}}
\end{table}



\begin{figure}
\begin{minipage}[l]{0.3\textwidth}
\includegraphics[width=1\columnwidth]{figures/subreddit_distribution.png} 
\end{minipage}
\begin{minipage}[l]{0.3\textwidth}
\caption{\textbf{Misinformation, Toxicity, and Political Polarization Interactions}--- As subreddits increase in misinformation levels, they become more toxic. There is not a large correlation between misinformation levels and the political polarization of subreddits.}
\end{minipage}
\label{figure:subreddit_interaction}
\end{figure}


\begin{table}[b]
\centering
\begin{tabular}{lll}
\toprule
   \multicolumn{3}{c}{\large Number of Comments on Misinfo Submissions}          \\
   \toprule
                                  & {Zero Inflated}  & {Negative Binomial }  \\
                      &       \footnotesize{negative coefficient = } &  \footnotesize{positive coefficient = }\\
                      &       \footnotesize{more likely to get comments} &  \footnotesize{more comments}\\
      \midrule
      Intercept              & 5.810*** & 3.290***  \\               
      \midrule
      Absolute User Polarization               & -7.515***  & -3.550***  \\
      \midrule
      Absolute Subreddit Polarization              & 2.700*** &-0.568* \\
    \midrule
       Subreddit Toxicity & -6.395***   & 5.525*** \\
      \midrule
       User Toxicity &   -13.470*** &  -11.750***\\
      \midrule
      Average Subreddit Comments &  -9.112*** & 1.300***  \\
\bottomrule
& $^\ast p<0.05; \;  ^{**} p<0.01; \; ^{***}p<0.001$ \\

\end{tabular}
\end{table}


\begin{table}[b]
\centering
\begin{tabular}{lll}
\toprule
   \multicolumn{3}{c}{\large Number of Comments on Mainstream Submissions}          \\
   \toprule
                            & {Zero Inflated}  & {Negative Binomial }  \\
                      &       \footnotesize{negative coefficient = } &  \footnotesize{positive coefficient = }\\
                      &       \footnotesize{more likely to get comments} &  \footnotesize{more comments}\\
      \midrule
      Intercept              & 3.054***  &2.436*** \\               
      \midrule
     Absolute User Polarization               & -4.463***  & -2.566***  \\
      \midrule
      Absolute Subreddit Polarization              & 4.296*** &0.415 *** \\
    \midrule
      Subreddit Toxicity & 5.298***  & 12.033*** \\
      \midrule
       User Toxicity &   -12.261*** &  -7.558***\\
      \midrule
      Average Subreddit Comments &  -7.712*** & 0.861***  \\
\bottomrule
& $^\ast p<0.05; \;  ^{**} p<0.01; \; ^{***}p<0.001$ \\
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{lrrr}
\toprule
   SEVERE\_TOXICITY \\
   Threshold &   Precision &  Recall  &    F1-Score  \\ \midrule
      0.1  &0.307& 0.576 & 0.400\\
      0.2 &0.414 & 0.390 &0.401 \\
      0.3& 0.484 & 0.295 & 0.367 \\
      0.4 & 0.619 &  0.130 & 0.215 \\
      0.5 & 0.759 & 0.037 & 0.070\\
      0.6 & 0.774 & 0.010 &0.020\\
      0.7 & --- & --- & ---\\
      0.8 & --- & --- &---\\
      0.9 & --- &----& ----\\
\end{tabular}
\caption{Precision, Recall, and F-1 Scores of Perspective API's TOXICITY and SEVERE TOXICITY classifier in correctly labeling social media comments from Deepak et al.~\cite{kumar2021designing}'s dataset as toxic. }
\label{tbl:ergm}
\end{table}

\begin{tabular}{lrrr}
\toprule
TOXICITY \\
    Threshold &   Precision &  Recall  &    F1-Score  \\         \midrule
      0.1  &0.136& 0.991 & 0.240\\
      0.2 &0.152 & 0.975 &0.263 \\
      0.3&0.168 & 0.944 & 0.285 \\
      0.4 & 0.193&  0.841 & 0.314 \\
      0.5 & 0.222 & 0.692 & 0.337\\
      0.6 & 0.254 & 0.533 &0.344\\
      0.7 & 0.308 & 0.345 & 0.325\\
      0.8 & 0.402 & 0.185 &0.254\\
      0.9 & 0.594 &0.075& 0.133\\
      
\end{tabular}

\begin{figure}
\begin{minipage}[l]{0.8\textwidth}
\includegraphics[width=1\columnwidth]{figures/std_user_mentions.png} 
\end{minipage}

\begin{minipage}[l]{1\textwidth}
\caption{Users in the political center have the highest \textbf{average toxicity} compared to users on the political ends.   \label{fig:toxicity-vs-polarization}}
\end{minipage}

\end{figure}
%Finally, to ensure that we properly capture the behavior of those that twee mainstream and misinformation on Twitter, we gathered 16,000 different accounts that tweeted mainstream/authentic news domains between September 5, 2022, and November 2, 2022, as well as another 18,000  accounts that tweeted a misinformation domain link between  September 5, 2022, and November 2, 2022,  as well.

\begin{table}[t]
\centering
\small
\begin{minipage}[l]{0.4\textwidth}
\begin{tabular}{lrrr}
\toprule
   SEVERE\_TOXICITY \\
   Threshold &   Precision   \\ \midrule
      0.1  &0.307\\
      0.2 &0.414  \\
      0.3& 0.484  \\
      0.4 & 0.619\\
      0.5 & 0.759\\
      0.6 & 0.774 \\
      0.7 & --- & \\
      0.8 & --- & \\
      0.9 & --- &\
\end{tabular}
\end{minipage}
\begin{minipage}[l]{0.4\textwidth}
\caption{Precision Peerspective API's TOXICITY and SEVERE TOXICITY classifier in correctly labeling social media comments from Deepak et al.~\cite{kumar2021designing}'s dataset as toxic. }
\end{minipage}
\label{tbl:ergm}
\end{table}


\begin{table*}
\centering
\scriptsize
%\fontsize{8.5pt}{10pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{\textwidth}{l|llrXr}
\toprule
Topic &  {Keywords} & \# Tweets &  \# Toxic Tweets & Example Tweet  & Approx. Part. & Approx. Part. of Toxic\\ \midrule


 3 & putin,russia,ukraine,war,civilian  &1850209 & 18421  & RUSSIA FAILED. UKRAINE WON! Russia is destined to FAIL under maniacal Putin. It is a pariah among the world amp; its inhumane cruelty has been exposed: murdering civilians, raping women amp; children. What a collection of barbarians. Enemy of humanity. & -0.273 \\ %\hline



 1& republican, gop, demcorat, party,maga & 32,675 & Republicans are just disgusting, lying, no good, power grabbing, coward bastards! & -0.191 \\


  2 & block, fascist, asshole, bigot, post & 25,751 & @LieuColumbo @mattybones8 @realDailyWire @joerogan @jordanbpeterson Leave you alone? You really are a miserable person, aren’t you? I have tried to be nice. But, honestly? Go fuck yourself, buddy. We’re fucking through here & -0.112\\



  4 & nazi, hitler, jew, fascist, antisemite & 13,765 & Nazi punks fuc off!!! & -0.144 \\

  5 & racist, black, white, supremracist, color & 11,773 &  Hes a racist pig & -0.058 \\
 6 & dickhead, lol,bitf*cked, margin, f*ck & 10,873 &   Who is that asshole? & -0.017 \\

 7 & abort, baby, brith, unborn,proliferate & 10,272 & Until those little creatures can take the "breath" of life on their own, then it is up to WOMEN to decide what is to be done! Fuck you and you notions of patriarchal control of women\'s bodies. Until further notice we ARE the God in your life! & 0.146 \\

  8 & phedophilia, pedo, child, graphic,pervert & 9,130 &Ladies and Gentlemen the PedoDent of the United States $\#$PedoHitler & 0.235   \\

  9 & nigga, rap, aint, song, yo & 8,392 & I was so mad but I had to be cool. Cause bitches is really out here setting niggas up. And when you gotta street nigga, they gotta protect themselves all the time. & -0.066 \\


  10 & twitter, tweet,elon, retweet, musk & 7,284 &Twitter isnt a representative democracy and we dont give criminals and sociopaths representation when we are enjoying one. Which you already know, you disingenuous fuck. & -0.085 \\

\bottomrule
\end{tabularx}
\caption{\label{tab:narratives} Top toxic topics---by number of tweets---in our dataset.} %\todo{how was this selection made? Sounds vague.
\end{table*}


\begin{table*}
\centering
\scriptsize
%\fontsize{8.5pt}{10pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{\textwidth}{l|lrXr}
\toprule
Topic &  {Keywords} & \# Toxic Tweets & Example Tweet  & Approx. Partisanship\\ \midrule
 1& spy, china, bang, community,fang & 142 &You fucked a Chinese Communist Party spy.  You should probably just shut up, Corky.  & 1.000 \\
\bottomrule
\end{tabularx}
\caption{\label{tab:narratives} Top toxic topics  with at least 100 tweets and 10 users---by conservative tilt---in our dataset.} %\todo{how was this selection made? Sounds vague.
\end{table*}


\begin{table*}
\centering
\scriptsize
%\fontsize{8.5pt}{10pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{\textwidth}{l|lrXr}
\toprule
Topic &  {Keywords} & \# Toxic Tweets & Example Tweet  & Approx. Partisanship\\ \midrule
 1& spy, china, bang, community,fang & 142 &You fucked a Chinese Communist Party spy.  You should probably just shut up, Corky.  & 1.000 \\
2 & break, liar, idiot, scumbag,alert &268 &   @Breaking911 Piece of shit & 0.849 \\
3  & phedophile, chief, burn, dead, asshole &154 &  @ProudElephantUS Sl* u *t & 0.823 \\

4  & biden, joe, hell, hunter, die &213 & @BidensWins Fuck u Biden & 0.780\\
5 & rino, piece, rishi,sunak,worthless &236 & Fucking rino mother fucker!!!! & 0.778 \\
6  & fuck, hag, diseased, crazy, liberal &271  &@GioBruno1600 Piece of Shit!!' & 0.774 \\

7 & china, jihad, butt, biden, kiss & 140 & CHINA'S QUID PRO QUO JIHAD BUTT KISS PUPPET, BULLSHIT ARTIST JOE BIDEN...COMPLETE WITH DEMENTIA!!!& 0.767 \\

8  & schiff, schumer, adam,chuck, lie & 279 & @RepAdamSchiff Schiff is a lying evil scumbag!  & 0.758 \\
9  & baby, kill, womb,birth, unborn & 257 & URGENT: YOU CAN STILL KILL YOUR BABIES  & 0.750 \\
10  & jackson, ketanji, child, brown, porn & 108 & Kiddie Porn and Child Molester Problems the Big issue with Judge Ketanji Brown Jackson - Children Raped and Sodomized & 0.728 \\
\bottomrule
\end{tabularx}
\caption{\label{tab:narratives} Top toxic topics  with at least 100 tweets and 10 users---by conservative tilt---in our dataset.} %\todo{how was this selection made? Sounds vague.
\end{table*}


\begin{table*}
\centering
\scriptsize
%\fontsize{8.5pt}{10pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{\textwidth}{l|lrXr}
\toprule
Topic &  {Keywords} & \# Toxic Tweets & Example Tweet  & Approx. Partisanship\\ \midrule
 1& mr, rott, fuck, motherfuck,treason & 155 &@BaddCompani Fcuk that guy  & -1.15\\
 2& gay, death, facist, homophobe,asswipe & 201 &$\#$DeathSantis the Fascist& -1.13 \\
  3& white, racist, her, stupid,damn & 191 &@notcapnamerica She sounds like a whole ass idiot. He has killed children. Fuck him and her.& -1.03 \\

  4 & lie, fuck, guy, piece,idiot & 530 &@Acyn You. You fucking Nazi!& -1.00\\

  5 & gqp, nazi, party, homophobe,vote & 215 &@RBraceySherman 3/what pisses me off the most about bs like UR whiny privileged article is that Trump ; GQP did so much fucking damage…U all expect 1 election (an election where many failed 2vote in Dem at local level)…U expect a quick fix?! Stop whining ,attack GQP not Dems;fucking vote. !& -0.921\\

  6 & elise,bottom,feed,cheat,filthy & 342 &@EliseStefanik @seanhannity Batshit crazy @elisestafanik please just go crawl back under your porch and stay there.& -0.917\\
   7 & whore,hooker,dick,trash,douchebag & 342 &  @MysterySolvent Asswipe& -0.911\\

   8 & putin,ukraine,slava,thug,war & 131 & @olex\_scherba $\#$RussiaIsATerroristState& --0.907\\

   9 & marg,cult,guilty,violation,beat & 119 & @RepMTG You're so full of shit, Marge.& --0.883\\

   10 & cathowrn, cousin,madison, orgy, nazi &287 & @CawthornforNC fuck you, asswipe.  & -0.872 \\
\bottomrule
\end{tabularx}
\caption{\label{tab:narratives} Top toxic topics  with at least 100 tweets and 10 users---by liberal tilt---in our dataset.} %\todo{how was this selection made? Sounds vague.
\end{table*}


\begin{figure}
\begin{minipage}[l]{0.48\textwidth}
\includegraphics[width=1\columnwidth]{figures/toxicity_vs_cluster_std.png} 
\end{minipage}
\begin{minipage}[l]{0.48\textwidth}
\caption{As previously also found in our analysis of user characteristics (Section~\ref{sec:calculated}), we find that as users engage in a wider window of topics of particular political ideologies, the more toxic their tweeted content\label{fig:toxicity-vs-var}}
\end{minipage}

\end{figure}

% \subsection{Misinformation and Authentic News Dataset}

%To understand how users who utilize questionable sources on Twitter interact with other users, we first curate a list of websites that often publish unreliable and otherwise unverifiable information. As a control, we further gather a separate list of websites that publish reliable and verifiable information.  Specifically, we aggregate together unreliable and reliable news domains previously gathered by Iffy News,\footnote{\url{https://iffy.news/index}} OpenSources,\footnote{\url{https://github.com/several27/FakeNewsCorpus}} Politifact,\footnote{\url{https://www.politifact.com/article/2017/apr/20/politifacts-guide-fake-news-websites-and-what-they/}} Snopes,\footnote{\url{https://github.com/Aloisius/fake-news}} and Melissa Zimdars\footnote{\url{https://library.athenstech.edu/fake}}, Hanley et~al.~\cite{hanley2022golden}, and MediaBias/FactCheck. We note for MediaBias/FactCheck that we father our set of  unreliable news domains from the set of websites labeled as ``questionable sources''; similarly we gathered our set of reliable websites from those labeled as center-right, center-left, and center. Altogether, we collect a total of 1,376 unreliable news domains and 2,285 reliable news websites. Our list of misinformation domains included websites such as globalresearch.ca, infowars, and thegatewaypundit.com which have been documented as being parts of toxic political echo-chambers~\cite{starbird2018ecosystem}. Our list of reliable news domains consists of websites across the political including foxnews.com, dailywire.com, nytimes.com, and cnn.com.




 %Lastly, we note that. %Altogether we gather

% In addition to this core dataset, we also utilize the Twitter Streaming API to understand the larger Twitter ecosystem and the relative toxicity and amounts of misinformation on the platform. The Twitter Streaming API gives real-time access to 1\% of public tweets. We continuously collected these tweets between July 10 and December 21, 2022. We utilize this dataset to understand the characteristics of English-language Twitter. 






%As found by Kumar~\textit{et al.}~\cite{kumar2021designing}, utilizing this particular classifier at a threshold of 0.6~\cite{kumar2021designing}, provides an acceptable precision for identifying toxic online content across different subgroups of users. Throughout this work, we thus consider a tweet as toxic if as a SEVERE\_TOXICITY score above 0.6.

\begin{figure}
\begin{minipage}[l]{0.8\textwidth}
\includegraphics[width=1\columnwidth]{figures/user_toxicity_vs_partisanship.png} 
\end{minipage}

\begin{minipage}[l]{1\textwidth}
\caption{Users in the political center have the highest \textbf{average toxicity} compared to more liberal or conservative users. \label{fig:toxicity-vs-polarization}}
\end{minipage}

\end{figure}


\begin{figure}
    \centering
\begin{minipage}[l]{0.6\textwidth}
\includegraphics[width=1\columnwidth]{figures/all_vs_toxic_political_mentions.png} 
\end{minipage}
\begin{minipage}[l]{0.33\textwidth}
\caption{ When users mention (@) users that are more politically different than themselves, they are more likely to be toxic. On average Toxic Tweets  (SEVERE\_TOXICITY> 0.3) occur in mentions with more disparate political ideologies compared to all tweet interactions.  \label{fig:politican-diff-toxicity}}
\end{minipage}
\end{figure}



\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{lrrr}
\toprule
   SEVERE\_TOXICITY \\
   Threshold &   Precision &  Recall  &    F1-Score  \\ \midrule
      0.05 & 0.284 & 0.624 & 0.390 \\  
      0.10  &0.307& 0.576 & 0.400\\
      0.15 & 0.321&0.543 & 0.404 \\
      0.20 &0.414 & 0.390 &0.401 \\
      0.25& 0.466 & 0.311& 0.373 \\
      0.30& 0.484 & 0.295 & 0.367 \\
      0.35& 0.530 & 0.246 & 0.336 \\
      0.40 & 0.619 &  0.130 & 0.215 \\
      0.45 & 0.651 &  0.099 & 0.172\\
      0.50 & 0.759 & 0.037 & 0.070\\
      0.55 & 0.766 & 0.015 & 0.029\\
      0.60 & 0.774 & 0.010 &0.020\\
      0.65 & --- & ---  &--- \\
      0.70 & ---  & ---  &--- \\
       0.75 & ---  & ---  &--- \\
       0.80 & ---  & ---  &--- \\
       0.85 & ---  & ---  &--- \\
       0.90 & ---  & ---  &--- \\
\end{tabular}
\begin{tabular}{lrrr}
\toprule
   TOXICITY \\
   Threshold &   Precision &  Recall  &    F1-Score  \\ \midrule
      0.05 & 0.129 & 0.996& 0.228 \\  
      0.10  &0.136& 0.991 & 0.239\\
      0.15 & 0.144&0.984 & 0.251 \\
      0.20 &0.152 & 0.975 &0.263 \\
      0.25& 0.159 & 0.965& 0.272\\
      0.30& 0.168 & 0.944 & 0.285 \\
      0.35& 0.179 & 0.908 & 0.300 \\
      0.40 & 0.193 &  0.841 & 0.314 \\
      0.45 & 0.208 &  0.771 & 0.327\\
      0.50 & 0.222 & 0.693 & 0.336\\
      0.55 & 0.234 & 0.617 & 0.343\\
      0.60 & 0.254 & 0.533 &0.344\\
      0.65 & 0.279 & 0.432 &0.339\\
      0.70 & 0.308 & 0.345 &0.325\\
       0.75 & 0.336 & 0.281 &0.306\\
       0.80 & 0.402 & 0.186 &0.254\\
       0.85 & 0.466 & 0.137 &0.211\\
       0.90 & 0.594 & 0.075 &0.133\\
\end{tabular}
\caption{Precision, Recall, and F-1 Scores of Perspective API's TOXICITY and SEVERE TOXICITY classifier in correctly labeling social media comments from Kumar et~al.~\cite{kumar2021designing}'s dataset as toxic.}
\label{tbl:perspective-f1}
\vspace{-15pt}
\end{table}


\begin{table}
    \small
    \centering
    \begin{tabularx}{0.7\columnwidth}{l|lrr}
    \toprule
  Adjusted R-squared:  0.373  & Coefficient  & Std. Error & Adj. Sum Sq. \\    \midrule
  Intercept &${-0.108}^{***}$& 0.012 & 0.983\\
  Log \# Users & $-0.005$ & 0.003 &0.029 \\
  Percentage Verified & $0.040$& 0.020 & 0.015 \\
  Avg User Toxicity in Cluster & $\textbf{2.897}^{***}$ & 0.065 & \textbf{16.95} \\
 Abs Cluster Political Ideology  & $-0.093^{***}$ & 0.015  & 0.352\\
 Std Cluster Political Ideology  &  $0.0415^{***}$ & 0.010 &0.072	\\
  Left/Right  & 0.0054& 0.003 &0.026\\
    \bottomrule
     \multicolumn{4}{c}{ $^\ast p<0.05; \;  ^{**} p<0.01; \; ^{***}p<0.001$ }
    \end{tabularx}
  \caption{Linear fit on factors in the toxicity in individual topic clusters. } 
   \vspace{-15pt}
   \label{table:regression-cluster-toxicity}
\end{table}

\begin{table*}
\centering
\scriptsize
%\fontsize{8.5pt}{10pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{\textwidth}{l|XrrrXrrr}
\toprule
 &   &  &   \# Toxic  & Avg.& Example & Avg.  & Avg. Partisan  & Partisan \\
 Topic& {Keywords}&\# Tweets & Tweets & Toxicity &  Tweet  & Partisan. & of Toxic Users& Std. \\

\midrule
1 & mastriano, thanmaga, antisemitic, louder, mastribator & 128& 74 (57.82\%) &0.492 & Sen Mastriano You're an anti-Semitic POS.
 & -2.176& -0.682 & 1.791 \\
 2& delta, operator, fking, dawn, nightclub & 284 & 89 (31.34\%)& 0.321 &I Have To Kill This Guy Before He Kills Us:' Army Vet Says After Harrowing Nightclub Shooting & 1.034& 0.152 & 1.693 \\

 3 & defeatist, sore, winning, lose, metabolize, & 476 & 127 (26.68\%) & 0.270&Same hypocrites who say the losers should lose gracefully on the very rare occasion they actually win anything. & -0.586 &-0.152 & 1.548 \\

4 & scalise, saved, steve, trumpshit, sleazy & 246 & 65 (26.42\%)& 0.282 & EWhen bringing up that Steve Scalise was also attacked can we also bring up the fact it was a gay black woman who saved his ass & -0.565 &-0.900& 1.548 \\

5 & tillis, thom, burr, nc, sen, establishment & 2,199&271 (12.32\%)& 0.143 & Sen Thom Tillis Traitor 
You've always been a RINO
NC must be ashamed of you  & 0.049 & 0.372 & 1.424 \\
 
\bottomrule 
\end{tabularx}
\caption{\label{tab:variance-topics} Top toxic topics by variation in user partisanship.} 
\vspace{-10pt}
\end{table*}

==> engagement.tex <==
\section{RQ3: Engagement with Misinformation and Authentic News}
Having explored how misinformation on Reddit promotes toxic, insular, and polarized environments on Reddit, we finally turn to understand these factors' role in user engagement with misinformation and authentic news.  Namely having seen that misinformation produces more toxic and politically uncivil environments, do these environments lead to more engagement with misinformation? Various works have found that toxic and polarized environments often provoke engagement from users as they get ``outraged'' by the presented content~\cite{kim2021distorting,gallacher2021online}. In this final section, we seek to determine how different communities and different community norms affect the rates at which misinformation and authentic news get interactions on Reddit.

\subsection{Experimental Setup} To understand user interactions and engagement with misinformation and authentic news URL submissions, we utilize the number of comments that each submission receives. We utilize the number of comments rather than the number of upvotes/downvotes, due to the unreliability of Pushshift's data for this particular submission characteristic. While Pushshift often can acquire most submissions and comments, it often fails to keep up-to-date information about the number of votes a given submission receives~\cite{baumgartner2020pushshift}. This is largely due to the high rate at which submission upvotes/downvotes change. We thus use the more stable and reliable ``number of comments'' number to determine user engagement with a given submission. We lastly note that to properly model the number of comments, we remove comments from Reddit ``auto moderator'' accounts (often subreddits have auto moderators that automatically comment on submissions). We thus consider the number of comments from ``real world'' users. 

\begin{figure}
\begin{minipage}[l]{0.4\textwidth}
\includegraphics[width=1\columnwidth]{figures/num_submissions.png} 
\end{minipage}
\begin{minipage}[l]{0.35\textwidth}
\caption{\textbf{Log of number of submissions for misinformation and authentic news submissions}--- A large majority of submissions do not receive  comments.\label{fig:num_comments}}
\end{minipage}

\end{figure}


To model the count data of the number of comments on given submissions, we utilize a zero-inflated negative binomial regression~\cite{ridout2001score}. Within our regression, each observation represents a single submission and the number of comments it garnered. We specifically utilize a zero-inflated negative binomial regression as it appropriately models our set of count data. Unlike a Poisson model, which is often utilized to model count data, negative binomial regressions do not make the strong assumption that the mean of the data is equal to the variance~\cite{morina2022web}. Given that some submissions garner thousands of comments while others garner none, utilizing a Poisson model would be somewhat inappropriate. We further utilize the zero-inflated version of this regression given the heavy preponderance of submissions that do not receive any comments. After removing comments from auto moderators, as depicted in Figure~\ref{fig:num_comments}, 54.5\% of submissions within our dataset did not receive any comments. A normal negative binomial model would thus be unable the correctly model this behavior. 

\begin{table}[b]
\centering
\begin{tabular}{lll}
\toprule
   \multicolumn{3}{c}{\large Number of Comments on Misinfo Submissions}          \\
   \toprule
                                  & {Zero Inflated}  & {Negative Binomial }  \\
                      &       \footnotesize{negative coefficient = } &  \footnotesize{positive coefficient = }\\
                      &       \footnotesize{more likely to get comments} &  \footnotesize{more comments}\\
      \midrule
      Intercept              & 5.3146*** & 3.290***  \\               
      \midrule
      Absolute User Polarization               & -7.2400***  & -4.5838***  \\
      \midrule
      Absolute Subreddit Polarization              & 5.3818 &0.9658** \\
    \midrule
       Subreddit Toxicity & -2.5780***   & 5.3042*** \\
      \midrule
       User Toxicity &   -11.3991  *** &  -11.8022***\\
      \midrule
      Average Subreddit Comments &  -7.0379 *** & 1.0354***  \\
\bottomrule
& $^\ast p<0.05; \;  ^{**} p<0.01; \; ^{***}p<0.001$ \\
\end{tabular}
\caption{Fit of our zero-inflated negative binomial regression on the number of comments on our set of misinformation URL submissions across different subreddits.} 
\label{tbl:misinfo-fit}
\end{table}
\begin{table}[b]
\centering
\begin{tabular}{lll}
\toprule
   \multicolumn{3}{c}{\large Number of Comments on Authentic News Submissions}          \\
   \toprule
                            & {Zero Inflated}  & {Negative Binomial }  \\
                      &       \footnotesize{negative coefficient = } &  \footnotesize{positive coefficient = }\\
                      &       \footnotesize{more likely to get comments} &  \footnotesize{more comments}\\
      \midrule
      Intercept              & 3.7182***  &2.7577*** \\               
      \midrule
     Absolute User Polarization               & -2.7390***  & -3.0487 ***  \\
      \midrule
      Absolute Subreddit Polarization              & 5.9227*** &1.4898 *** \\
    \midrule
      Subreddit Toxicity & 6.1866***  & 13.1317*** \\
      \midrule
       User Toxicity &   -14.8969*** &  --8.0695***\\
      \midrule
      Average Subreddit Comments &  -6.4304*** & 0.6121***  \\
\bottomrule
& $^\ast p<0.05; \;  ^{**} p<0.01; \; ^{***}p<0.001$ \\
\end{tabular}
\caption{Fit of our zero-inflated negative binomial regression on the number of comments on our set of authentic news URL submissions across different subreddits.} 
\label{tbl:mainstream-fit}
\end{table}
Zero-inflated negative binomial regressions return two sets of coefficients. One set of coefficients, the zero-inflated coefficients, estimated using logistic regression, give the probability that the given submission would receive 0 comments as a function of the covariates. Positive coefficients for these zero-inflated coefficients indicate that increases in the predictor variable make a receiving 0 comment more likely. Thus the more negative a coefficient, the more the given covariate correlates with inducing at least 1 comment. The second set of coefficients, the negative binomial coefficients, model the number of comments as a function of the covariates. For these coefficients, positive coefficients indicate that the larger the corresponding covariate, the more comments that submission was likely to have received.  We thus, in our analysis, can understand how different covariates affect the probability that a given submission will receive \textit{any} comments \emph{and} how these same covariates affect the number of comments received. 

For data, we model the number of garnered comments for both our set of 47,822 misinformation submissions and 787,603 authentic news submissions. As factors influencing the number of comments, we utilize (1) the submitter's polarization, (2) the subreddit's polarization, (3) the toxicity norm of the subreddit, (4) the submitter's toxicity norm, and (5) the average number of comments with the subreddit the submission was posted in. 


\subsection{Results}  Before engaging in a thorough analysis of the fits of our zero-inflated negative binomials, we first perform a spot-check on the results. We ensure that the higher the average amount of comments in a given subreddit the more likely a submission is to get comments and that this average correlates with more comments on given submissions. In other words, we check that submissions in subreddits where users comment more, also received more comments. As seen in both Tables~\ref{tbl:misinfo-fit} and~\ref{tbl:mainstream-fit}, for both misinformation and authentic news Reddit submissions as the average number of comments in a particular subreddit increases, (1) the more likely a submission is to get comments at all and (2) the more comments it is likely to get. Having observed this behavior, we now move to examine the rest of the covariates within our fits. 

\paragraph{User Polarization} We observe similar behavior for the effect of the posting user political polarization on the number of comments that the submissions received. For both authentic news and misinformation submissions, we see that as the submission's submitter becomes more politically polarized (\textit{i.e.} moves to the political extremes on the political left or right), the more likely their posts are to receive comments. With zero-inflated coefficients of -7.24 for misinformation submissions and -2.74 for authentic news submissions, we see that this is particularly true for misinformation submissions. This largely agrees with prior work that has shown that highly polarized users are likely to provoke and garner comments on social media platforms~\cite{kim2021distorting,howard2019ira}

However, despite highly polarized users being able to attract at least one comment, we further observe that for both authentic news and misinformation submissions as the posting user becomes more politically polarized, the fewer comments their post is likely to receive. This appears to indicate that in the case of misinformation and authentic news submission, Reddit users are perhaps being ``turned off'' and engaging less with highly polarized users~\cite{hetherington2008turned}compared to more politically neutral users.

\paragraph{Subreddit Polarization} While we are unable to conclude using our model whether subreddit polarization has an effect on misinformation submissions, we find that for authentic news submissions the more politically polarized a subreddit is, the less likely anyone is to comment on authentic news submissions. This may indicate as a whole that authentic news submissions do not ordinarily get much traction on highly polarized subreddits. Rather, as documented by Wang \textit{et al.}~\cite{wang2021multi} subreddits like these often ignore more trustworthy sources. We thus find that the insular nature of more partisan subreddits may be inducing them to largely ignore authentic news submissions when they appear within their subreddit.
 
In contrast, for both misinformation and authentic news submissions, we find that as polarization goes up, the more comments given submissions are likely to garner. This reflects that \emph{when} authentic news and misinformation submissions are noticed, the more polarized the environment, the more users seem to comment and engage with submissions~\cite{kim2021distorting}.
 
\paragraph{Subreddit Toxicity}
Looking at the subreddit toxicity, we see a marked difference between authentic news submissions and misinformation submissions. We see, notably, for misinformation submissions, the more toxic a subreddit is, the more likely the submission is to get comments. In contrast, for authentic news submissions, the more toxic the subreddit, the more likely the submission is to not get any comments at all. This appears to reflect that authentic news submissions may often not have ``clickbait'' titles that induce readers to often angrily engage with  material~\cite{chen2015misleading,potthast2016clickbait}. In contrast, oftentimes misinformation websites often post inflammatory articles designed to engender angst in their readership. For example, with regards to the COVID-19 pandemic, the misinformation website infowars.com~\cite{starbird2018ecosystem}  recently published a report entitled \textit{``Wake Up! Even The Masks Made You Sick''!} As subreddits get more toxic, we thus see that their users are more likely to engage with articles such as this. 
 
Similar to polarization, for both misinformation and authentic news submissions, we find that as subreddit toxicity goes up, the more comments given submissions are likely to garner. This again reflects that \emph{when} authentic news and misinformation submissions are noticed, the more toxic the environment the more users seem to comment and engage with submissions. We thus see that though authentic news submissions are more often ignored in toxic subreddits when compared to misinformation, when they are noticed, toxic environments produce more engagement with both types of submission. 

\paragraph{User Toxicity}  Finally, looking at user toxicity, we see similar behaviors for both authentic news and misinformation submissions. Most notably, as users become more toxic for both misinformation and authentic news submission, the more likely they are to provoke at least one comment. We thus see that user toxicity is a means by which to gain engagement from posting news articles generally. However, again in both cases, we see that while user toxicity often provokes at least one person to react, we see that this toxicity, often does not lead to more comments on the whole. As found in prior work, toxic users, while often sparking retorts as other users become enraged, also create unhealthy, short, and otherwise bad conversational outcomes~\cite{saveski2021structure,kumar2021designing}. This result largely matches our definition of individual toxicity as comments that \textit{are likely to make one leave the discussion} from Section~\ref{sec:misinformation-defintion}. We thus as a whole see that as entire communities/subreddit becomes more toxic, they are more likely to engage with materials more thoroughly, but as individual users become more toxic, they are more likely to end and otherwise shorten conversations. 








==> interactions.tex <==
\section{Reddit Level Interactions}
As found in prior work, subreddits maintain particular levels of toxicity community norms~\cite{rajadesingan2020quick}. For example, as found by Rajadesingan \textit{et al.}, the subreddit WhiteRights had much higher tolerance for toxic content than the subreddits NeutralPolitics or AskEconomics. In this section, we analyze how distinctive political norms and toxicity levels within given subreddits contribute to levels of misinformation. 


In order to get an approximation of the levels of misinformation within a given subreddit we utilize a set of 157,605 \textit{misinformation-oriented} websites. We define \textit{misinformation-oriented} websites as websites that have more connections from our set of misinformation websites than from authentic news (i.e., the majority of a site's inward links in a domain-based graph are from misinformation websites. Websites that have been widely documented as spreading falsehood and conspiracy theories are included within this list including InfoWars and 8kun.top~\cite{hanley2022no,starbird2018ecosystem}.


As seen in Figure~\ref{figure:misinfo-toxciity-polarization}, there are political and toxicity norms across the spectrum, with polarization levels not being correlated levels of toxicity nor with misinformation levels. We see in particular that subreddits that are at the edge of political spectrum actually have some of the lowest average Perspective Toxicity scores and the lowest amounts of misinformation hyperlinks. We thus see at that at the edges of the political spectrum, where users are more isolated and insular that the overall levels of toxicity within the subreddit are not as high as those more ``moderate'' subreddits. This suggests that these cohesive communities where users are more similar to each other may producing the least amounts of bad behavioral outcomes. 


As seen in Figure~{}, toxicity the


\begin{figure}
\centering
\includegraphics[width=0.75\columnwidth]{figures/subreddit_distribution.png} 
\caption{\textbf{Distributions of political polarization, perspective toxicity levels, and misinformation-oriented URL usage across subreddits with at least 100 users }--- While previous research has indicated that political polarization and toxicity are heavily correlated, we see in Reddit's case due to its self-selecting communities that political polarization is not correlated with vitriol and comment toxicity. Similarly we see that political polarization is not correlated with misinformation levels. Rather subreddits within the political center have the highest percentages of misinformation and toxicity. 
}
\label{figure:misinfo-toxciity-polarization}
\end{figure}

==> interplay.tex <==
\section{RQ2: Misinformation and Polarized Toxic Conversations}\label{sec:toxic-polarized-subreddits}
As seen in the previous section, comments are 60\% more toxic under misinformation submissions than authentic news submissions. Furthermore, there appears to be a difference in the political orientation of users that post misinformation and those that comment on it.  Given this difference and the higher toxicity levels present within misinformation submission comments, we now turn to understand if and how these \textit {political differences} drive toxicity within Reddit misinformation submissions. 

\subsection{Experimental Setup}
To fully understand how different levels of \textit{political differences} fuel toxicity and incivility, for this section, we reconstruct the conversational dyads that exist underneath each Reddit submission using the data provided by Pushshift~\cite{baumgartner2020pushshift}. Comments underneath Reddit submissions are similar to conversational threads; if a user responds to a given comment, their reply will appear underneath the comment. For each submission in our dataset, we thus determine using the thread information whether the commenter posted a response directly to another commenter. This then enables us to reconstruct conversational dyads between individual Reddit users. Then, using the approach outlined in Section~\ref{sec:reddit-methods}, we determine the polarization and average toxicity of the users in our conversational dyads. From these calculations, we further label users as conservative/conservative-leaning (positive polarization score) or liberal/liberal-leaning (negative polarization based). Lastly, looking at each of these conversational dyads, we determine if each user's response to each other is toxic/uncivil by utilizing the Perspective API SEVERE\_TOXICITY classifier with a cutoff of 0.8 (as also outlined in Section~\ref{sec:reddit-methods}). For a comparison of how conversations differ between misinformation and authentic news comments, we finally separate out the set of conversational dyads that appear under misinformation and authentic news submissions (for both sets of URLs). 
\begin{figure*}
\begin{subfigure}{.49\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/subreddit_interparty_interaction.png}

  \label{fig:pagerank-sub2}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/subreddit_mainstream_interaction.png}

  \label{fig:pagerank-sub2}
\end{subfigure}
\caption{\textbf{Proportions of inter-party interactions in different subreddits}---As subreddits hyperlink to more \textit{misinfo-oriented} websites, as a percentage, there are fewer and fewer interactions between conservative and liberal users. In contrast, there is a slight correlation between hyperlinking to \textit{mainstream-oriented} websites and more inter-party interactions. }
\label{fig:subreddit-misinformation-mainstream-similarity-interaction}
\end{figure*}




\subsection{Toxic Interactions within Misinformation and Authentic News Environments}
We find high amounts of homophily in interactions across our conversational dyads. Across all our conversational dyads, indeed 81.3\% of interactions are between users of the same political orientation (\textit{i.e} liberal-liberal, conservative-conservative). In contrast, for conversations under mainstream, and misinformation submissions, this increases to 81.7\% and 85.3\% respectively. We thus see slightly more conversational homophily within misinformation conversations than the entire Reddit population at large. Indeed using our set of \textit{misinfo-oriented} and \textit{mainstream-oriented} and looking at subreddits with at least 500 conversational dyads, as seen in Figure~\ref{fig:subreddit-misinformation-mainstream-similarity-interaction}, as website hyperlink to more \textit{misinfo-oriented} websites, conversations on their subreddits become more insular ($\rho =0.160$). In contrast, as subreddits hyperlink to more \textit{mainstream-oriented} websites, there is a slight increase in the amount of inter-party conversations ($\rho =0.153$). We thus see that misinformation is correlated with heightened political homophily within the subreddits, creating more insular communities, while authentic news is associated with a slight increase in political heterophily.

\begin{figure}
\centering
\begin{minipage}[l]{0.4\textwidth}
\centering
\begin{tikzpicture}[very thick]

    % Right square
    \node[fill=gray!20,draw=black, minimum size=1.2cm, inner sep=0pt] (as) {\footnotesize
$0.96\%$};
    \node[draw=black,minimum size=1.2cm, inner sep=0pt, above=-\pgflinewidth of as] (abh) {\footnotesize$0.91\%$};
    \node[draw=black,minimum size=1.2cm, inner sep=0pt, right=-\pgflinewidth of as] (abv) {\footnotesize$0.89\%$};
    \node[fill=gray!20,draw=black, minimum size=1.2cm, inner sep=0pt,  above right=-\pgflinewidth and -\pgflinewidth of as]  {\footnotesize$0.99\%$};
    
    % Side labels
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=0.7cm] at (as.west) {\scriptsize

Conservative};
    \node[anchor=north,] at (as.south) {\scriptsize
Liberal};
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=0.5cm] at (abh.west) {\scriptsize
Liberal};
    \node[anchor=north] at (abv.south) {\scriptsize
Conservative};
    
    
    % Square label
    \node[xshift=0.5cm, below=0.5cm of as] {\footnotesize Target};
    
    \node[yshift=1.0cm,xshift=-0.35cm,rotate=90,left=0.5cm of as] {\footnotesize Author};

\end{tikzpicture}
\end{minipage}
\begin{minipage}[c]{0.40\textwidth}
  \caption{\label{fig:interactions}\textbf{Percentage of interactions that are toxic/uncivil for authors and targets of different political leanings.} Across all 46K considered subreddits, there is a slight heterophily for users to reply in a toxic/uncivil manner to members with a tilt towards the opposite political party.}
\end{minipage}
\end{figure}    

Despite the increased political homophily within misinformation filled-subreddits, we observe a reverse trend in terms of toxic/uncivil comments. As seen in Figure~\ref{fig:interactions}, across all considered conversations, we see a slight heterophily for users to reply in a toxic/uncivil manner to users who are not of the same political leaning. We calculate an odds ratio of 1.17 for users to reply in a toxic manner to users of a different political leaning compared with users of the same political leaning. Comparing the set of toxic conversational dyads under misinformation submissions, we see an even higher heterophilic tendency. Compared with the baseline across all conversations, we observe a 25.2\% relative increase in the percentage of liberal to conservative toxic comments and a 12.5\% relative increase in the percentage of conservative to liberal toxic comments. In contrast, for authentic news submissions, we see a 23.2\% relative decrease in liberal to conservative toxic comments and an 18.8\% drop in the percentage of conservative to liberal toxic comments. This appears to indicate that while in misinformation-laced conversations, users are more likely to respond in a toxic manner to users of a different political orientation, users in authentic news-centered conversations are less likely.

To confirm, calculating the odds ratio we get 1.64 for misinformation toxic comments and  0.87 for mainstream toxic comments when comparing the percentages of politically heterophilic toxic comments to politically homophilic comments. Overall we thus find that on average, within misinformation submission comments that users are slightly more likely to respond with a toxic comment to users of different political leaning compared to all submissions on Reddit. This largely explains the higher levels of toxicity observed within misinformation submissions in Section~\ref{sec:toxicity} given the political differences we further observed between misinformation posters and misinformation comments.
 \begin{figure}
    \centering
    \begin{subfigure}{.4\textwidth}
       \centering
\begin{minipage}[c]{\textwidth}
   \centering
\begin{tikzpicture}[very thick]
    % Right square
    \node[fill=red!13,draw=black, minimum size=1.2cm, inner sep=0pt] (as) {\footnotesize$+12.5\%$};
    \node[fill=red!3,draw=black,minimum size=1.2cm, inner sep=0pt, above=-\pgflinewidth of as] (abh) {\footnotesize$+3.3\%$};
    \node[fill=blue!2,draw=black,minimum size=1.2cm, inner sep=0pt, right=-\pgflinewidth of as] (abv) {\footnotesize$-2.2\%$};
    \node[fill=red!25,,draw=black, minimum size=1.2cm, inner sep=0pt,  above right=-\pgflinewidth and -\pgflinewidth of as]  {\footnotesize$+25.2\%$};
    
   % Side labels
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=0.7cm] at (as.west) {\scriptsize

Conservative};
    \node[anchor=north,] at (as.south) {\scriptsize
Liberal};
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=0.5cm] at (abh.west) {\scriptsize
Liberal};
    \node[anchor=north] at (abv.south) {\scriptsize
Conservative};
    
    
    % Square label
    \node[xshift=0.5cm, below=0.5cm of as] {\footnotesize Target};
    
    \node[yshift=1.0cm,xshift=-0.35cm,rotate=90,left=0.5cm of as] {\footnotesize Author};


\end{tikzpicture}
\end{minipage}
   \caption{Misinformation Submission comments}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
\begin{minipage}[c]{\textwidth} 
   \centering
\begin{tikzpicture}[very thick]
    % Right square
    \node[fill=blue!19,draw=black, minimum size=1.2cm, inner sep=0pt] (as) {\footnotesize$-18.8\%$};
    \node[fill=blue!9,draw=black,minimum size=1.2cm, inner sep=0pt, above=-\pgflinewidth of as] (abh) {\footnotesize$-8.8\%$};
    \node[fill=blue!8,draw=blue!20,draw=black,minimum size=1.2cm, inner sep=0pt, right=-\pgflinewidth of as] (abv) {\footnotesize$-7.9\%$};
    \node[fill=blue!23,draw=black, minimum size=1.2cm, inner sep=0pt,  above right=-\pgflinewidth and -\pgflinewidth of as]  {\footnotesize$-23.2\%$};
  % Side labels
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=0.7cm] at (as.west) {\scriptsize

Conservative};
    \node[anchor=north,] at (as.south) {\scriptsize
Liberal};
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=0.5cm] at (abh.west) {\scriptsize
Liberal};
    \node[anchor=north] at (abv.south) {\scriptsize
Conservative};
    
    
    % Square label
    \node[xshift=0.5cm, below=0.5cm of as] {\footnotesize Target};
    
    \node[yshift=1.0cm,xshift=-0.35cm,rotate=90,left=0.5cm of as] {\footnotesize Author};

\end{tikzpicture}
 \caption{Authentic News Submission comments}
 \end{minipage} 
 \end{subfigure}
   \caption{Percentage increases of interactions that are toxic/uncivil in misinformation submissions for conservative and liberal authors against conservative and liberal targets.}
\end{figure}   

\subsection{Modeling toxic interactions between users commenting under Misinformation Submissions}
In order to confirm the finding that users of different political stripes in misinformation-laced conversations are more likely to reply in a toxic manner to each other, we fit our network data of toxic interactions to an exponential random graph model (ERGM). Exponential Random Graph Models (ERGM) is a form of modeling that predicts connections (toxic interactions) between different nodes (users) in a given network~\cite{hunter2008ergm}. ERGM models assume that connections are determined by a random variable $p^*$ that is dependent on input variables. As in Chen \textit{et al.}~\cite{chen2022misleading} and Peng \textit{et al.}~\cite{peng2016follower}, we utilize this modeling as it does it does not assume that its data input is independent; given that we want to model the interactions of polarization, toxicity, this relaxed restriction is key (we have already seen that they are largely not independent)~\cite{van2019introduction,hunter2008ergm}. Utilizing this framework, we thus model the probability of toxic interactions between a given author and target within misinformation submissions as a function of 1) their percentage of toxic comments, 2) their political polarization, 3) the difference in the author and target's political polarization 4) reciprocity between the author and target (\textit{i.e.} if the author and target both had a toxic comment aimed at each other), and finally 5) the number of subreddits that they share. 
\begin{table}[b]
\centering
\begin{tabular}{lr}
\toprule
   \multicolumn{2}{c}{\large Toxic Misinformation Submission Interactions}          \\
   \toprule
   & Coefficeint \\
      \midrule
      Intercept               &***-8.530 \\               
      \midrule
     Absolute User Polarization       &         -0.464 \\
      \midrule
      User Polarization Differences     & ***-0.782 \\
    \midrule
       User Toxicity &   ***12.396\\
      \midrule
       Reciprocity &  ***4.568\\
      \midrule
       Shared Subreddits &  0.00051\\
\bottomrule
 $\quad\quad\quad\quad ^\ast p<0.05; \;  ^{**} p<0.01; \; ^{***}p<0.001$ \\
\end{tabular}
\caption{As confirmed in our ERGM, differences in political orientation of users is predictive of increased incivility and toxicity. Similarly, the higher each individual user's toxicity norm they are more likely to target other users with toxic comments. }
\label{tbl:ergm}
\end{table}

Fitting our ERGM, we indeed find that as users become more politically distinct from each other, the more likely they are to target each other with uncivil or toxic comments (negative coefficient implies heterophily). As seen in Table~\ref{tbl:ergm}, political polarization by itself does explain toxicity as found by our model; rather differences between users seem to promote toxicity. This largely reinforces are findings from Section~\ref{sec:rq1}. Similarly, as expected, we find that higher levels of user toxicity norms and reciprocity between users are predictive of an increased probability of engaging in toxic interactions. We do not find as users share more subreddits that they are more likely to engage in toxic interactions with each other. 
We thus have seen that not only do misinformation submissions have more insular conversations, with 85.3\% of conversational dyads between users of the same political orientation (compared to 81.3\% of conversations under all Reddit submissions) but also that users become more hostile to users of the opposing political orientation.

\begin{figure*}
\begin{subfigure}{.49\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/subreddit_misinformation_interparty.png}
\label{fig:misinformation-interparty}
\end{subfigure}%s
\begin{subfigure}{.49\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/subreddit_misinformation_intraparity_toxicity.png}
  \label{fig:misinformation-intrapary}
\end{subfigure}

\caption{\textbf{Subreddit misinformation similarity vs. probability of toxic interactions between users of different and same political orientation}--- While for both inter-political and intra-political interactions, as misinformation similarity in a subreddit increases, the probability of a toxic interaction increases, for inter-political interactions the rate of increase is nearly double. }
\label{fig:subreddit-misinformation-rate-toxictiy-rate}
\end{figure*}


\subsection{Misinformation and increased rates of inter-political toxicity}
Finally, having confirmed that users posting under misinformation submission of different political orientations are more likely to engage in negative interactions with each other, we finally determine if the levels of misinformation within given subreddits as a whole leads to increased heterophilic toxic interactions. Namely as misinformation levels in a subreddit as a whole increase does the probability of negative interactions between users of different political orientations increase. We thus now plot the percentage of misinformation within a given subreddit against the probability of toxic interaction between members of the two political orientations. 


As seen in Figure~\ref{fig:subreddit-misinformation-rate-toxictiy-rate} looking at subreddits with more than 500 conversational dyads, we see that as subreddits have more \textit{misinformation-oriented} hyperlink submissions, the percentage of conversations dyads between users of different political leanings increases. Concretely, subreddit \textit{misinformation similarity} and the probability with which inter-political conversations are toxic have a correlation of $\rho=0.452$. While we similarly see that intra-political toxicity also increases with a similar correlation $\rho=0.447$, we see the rate at which misinformation induces inter-political toxicity is nearly 2.3 times that of intra-political toxicity (0.060 slope vs 0.026 slope). This reflects the fact that \textit{misinformation oriented} submissions are on the whole more toxic but that they increase politically heterophilic toxicity more than politically homophilic toxicity. 
\begin{figure*}
\begin{subfigure}{.49\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/subreddit_mainstream_toxicity_interparty.png}
\label{fig:misinformation-interparty}
\end{subfigure}%s
\begin{subfigure}{.49\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/mainstream_intra_party_toxic.png}
  \label{fig:misinformation-intrapary}
\end{subfigure}

\caption{\textbf{Subreddit misinformation similarity vs. probability of toxic interactions between users of different and same political orientation}--- For both inter-political and intra-political interactions, as mainstream similarity in a subreddit increases the probability of inter- and intra-political toxicity is largely flat.}
\label{fig:subreddit-mainstram-rate-toxictiy-rate}
\end{figure*}

Again comparing against subreddit mainstream similarity, we do not see a similar relationship. As seen in Figure~\ref{fig:subreddit-mainstram-rate-toxictiy-rate}, the relationship between inter-political and intra-political toxicity rates and similarity to mainstream sources is largely flat. 


\subsection{Summary} Misinformation, we find, not only promotes higher levels of toxicity in general but also appears to drive inter-political incivility. Fitting an ERGM to our misinformation toxic dyads, we indeed find that political differences (along with reciprocity and each user's toxicity) are a driving force behind the formation of a toxic conversational thread. Finally, examining how different levels of misinformation promote toxicity among users, we find that across our considered subreddits, misinformation drives inter-political incivility at 2.3 times the rate of intra-political toxicity. 





















 





%We now seek gain an understanding of whether Reddit subreddits where the misinformation URLs  were posted or the users commenting in the submissions themselves were driving the toxicity within the misinformation submissions. As seen in Figure~\ref{}, misinformation subreddits in both 



    
































==> reddit.tex <==
\section{Moderating Influences: Community Based Control on Misinformation Spread}
In this section, we examine the different misinformation ecosystems on Reddit. Largely in contrast to the self-organizing and porous communities that exist on Twitter, Reddit allows users to  establish their own self-contained communities. These communities known as subReddits have their own rules, communities norms, political preferences, as well as purposes. These subReddits module, control, and filter the content on Reddit platform. Behaviors in one subReddit that blocked or condemned in one subReddit can be widely celebrated in another subReddit. For example, one subReddit \texttt{r/conspiracy} that has over 1.7M (at time of writing in February 2022)  is dedicated to the discussion on conspiracy theories. Conspiracy Theories that are widely discussed in this subReddit are often ridiculed in other subReddit like \texttt{r/Qult\_Headquarters}.
\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/average-toxicity-end-2020.png}
\label{fig:cdf-subreddit-hyperlinks}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/average-toxicity-distribution-end2020.png}
 \label{fig:cdf-user-hyperlinks}
\end{subfigure}
\label{fig:cdf-hyperlinsk}
\caption{\textbf{Relative Perspective API toxicity of tweets and comments on Twitter and Reddit}--- Comparing a 1\% Twitter stream's Perspective API toxicity scores to the bulk of Reddit comments from  July to December 2020, we see that Reddit has maintained lower levels of toxicity over time and amongst users. }
\end{figure*}


\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/polarization_redidit_twitter.png}
\label{fig:cdf-subreddit-hyperlinks}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/average-toxicity-distribution-end2020.png}
 \label{fig:cdf-user-hyperlinks}
\end{subfigure}
\label{fig:cdf-hyperlinsk}
\caption{\textbf{Relative Perspective toxicity of tweets and comments on Twitter and Reddit}--- Comparing a 1\% Twitter stream's Perspective API toxicity scores to the bulk of Reddit comments from  July to Decemebr 2020, we see that Reddit has maintained lower levels of toxicity over time and amongst users. }
\end{figure*}
As seen in Figures~\ref{}

Because of self-organizing and fairly norm-heavy communities form on Reddit, we find that our set of misinformation URLs are largely confined to a small set of subReddits and set of users. As seen in Figure~\ref{fig:cdf-subreddit-hyperlinks}, fairly few subReddits are responsible for the amount of Misinformation URLs Reddit Submissions. For instance, we find that only 133 Reddits were responsible for 90\% of Misinformation URL submission on Reddit from July 2020 to December 2020. Only 4007 contained misinformation URLS within their submissions. 4878 different subReddits contained misinformation URLs in their comments.While some of misinformation posts could have been removed by moderators and Reddit itself, this illustrates the moderating effect community norms have on the material that is posted and stays posted in  the majority of subreddits. This is largely in contrast to the number of subReddits containing authentic news URLs, with 513 subReddits containing 90\% of authentic news URL submissions and 12,825 containing authentic news Reddit Submissions. 18131 different subReddits had authentic news domain hyperlinks in their comments from July 2020 to December 2020. This behavior among subreddits largely caries over to the set of Reddit users who posted these links to misinformation and authentic news websites. As seen in Figure~\ref{fig:cdf-user-hyperlinks}, just 1423 users were responsible for 90.0\% of of misinformation URLs subReddit submissions in contrast to the 11,336 responsible for authentic news submissions. 
\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/misinformation-authentic-cdf.png}
  \caption{\textbf{CDF News Hyperlinks by Subreddit}— Just 133 subreddits posted  90.0\% of hyperlinks to the misinformation websites in our dataset from July 2020 to December 2020. In contrast, 513 subReddits posted 90.0\% of the hyperlinks to authentic news websites during this same period. 
}
\label{fig:cdf-subreddit-hyperlinks}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/misinformation-authentic-users-cdf.png}
 \caption{\textbf{CDF News Hyperlinks by User}— Just 1423 subreddits posted  90.0\% of hyperlinks to the misinformation websites in our dataset from July 2020 to December 2020. In contrast, a whopping 11,336 subReddits posted 90.0\% of the hyperlinks to authentic news websites during this same period. 
}
 \label{fig:cdf-user-hyperlinks}
\end{subfigure}
\label{fig:cdf-hyperlinsk}
\end{figure*}


\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/partisanship_avg.png}
 
\label{fig:partisanship-average}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/toxicity_avg.png}
 
 \label{fig:toxicity-average}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/partisanship_variance.png}
 
\label{fig:partisanship-variance}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/toxicity_variance.png}
 
 \label{fig:toxicity-variance}
\end{subfigure}
\caption{\textbf{Toxicity and Political URL Variation among Users and SubReddits }--- As seen above, there are relatively tight windows of political partisanship and toxicity among subreddits with subreddits having approximately little more diversity than individual users. 
}
\label{fig:diversity-of-views}
\end{figure*}
\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/numberOfSubRedditsByPartianshipAvg.png}
  \caption{\textbf{User SubReddit Paritipation vs Variance in Political URLs Posted}-
}
\label{fig:participation-political}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/numberOfSubRedditsByToxicityAvg.png}
 \caption{\textbf{User SubReddit Paritipation vs Variance in Comment Toxicity}— 
}
 \label{fig:participation-toxicity}
\end{subfigure}
\caption{\textbf{Relative amounts of partisanship and toxicity diversity among individual users by SubReddit participation }--- As users participate in more and more the variance of their behavior increases with user posting a wider variety of political websites and commenting with a wider berth of toxicity. 
}
\label{fig:participation}
\end{figure*}
The moderating effect of subReddits is further seen in the relatively narrow window of political views and level of toxicity that are allowed within each subReddit community. As seen in Figure~\ref{fig:diversity-of-views}, there relatively narrow windows of allowed divergence in political beliefs and toxicity among SubRedits and users. This is in Figure~\ref{fig:participation}, as only as users participate in more and more subReddits does the berth of different types of comments that they post increase. On average, after a user participates in TODO subreddits the variance of their toxicity exceeds the average subReddit (an entire community). This illustrates the ability of subReddit communities to maintain an equilibrium of acceptable toxicity on their platforms, excising redditors who go outside normal bounds as illutrated in prior work~\cite{rajadesingan2020quick}.  Similarly, we find  that as users participate and post in more subReddits, they post a wider political range of websites.


\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/user-partisanship-var.png}
  \caption{\textbf{Number of SubReddit Users vs Variance in Political URLs Posted}-
}
\label{fig:participation-political}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/user-toxicity-var.png}
 \caption{\textbf{Number of SubReddit Users vs Variance in Comment Toxicity}— 
}
 \label{fig:participation-toxicity}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/partisanship-to-num-subreddits.png}
 
\label{fig:particiption-median-toxicity}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/toxicity-to-num-subreddits.png}

 \label{fig:cdf-user-hyperlinks}
\end{subfigure}
\label{fig:cdf-hyperlinsk}
\caption{\textbf{Number of Users to Variance in SubReddit Behavior}--- As the number of users in a particular subReddit increases, there is no discernible trend in the the variance of political URLS posted nor the Perspective API toxicity. However, as the the number of subReddits that the median user participates in increases within a given subReddit, the variance in political URLs and the the variance in toxicity does increase.  
}
\label{fig:participation}
\end{figure*}

Conversely, we find that the number of users that a subReddit contains, does not correlate with the diversity of toxicity and political views present on that subReddit. As seen in Figure~\ref{fig:participation}, as the number of users that post submissions in a subReddit increases, there is no discernible correlation with the variance of toxicity nor the variance of political views voiced on that subReddit. In contrast, we find that as the median subReddit participation on Reddit increases, the variance of toxicity and political viewd does increase.  Namely, if a subReddit has users that participate in a wide range of subReddits outside that particular subReddit, then this particular subReddit has higher levels of variance in political views and toxicity. This suggests that amount of people that a subReddit does not correspond with diversity of views and behavior on that subReddit but rather with the amount of communities that that subReddit's users come from and with which they engages. 
\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/user-misinfo-toxicity.png}
\label{fig:user-misnformation}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/reddit-misinfo-toxicity.png}
 \label{fig:reddit-misinformation}
\end{subfigure}
\label{fig:misinformation-reddit-user}
\end{figure*}
Having established how the characteristics of subReddits exerts norms over their particular users, we now turn to understand how these norms affect the levels of misinformation on Reddit platform and on particular subReddits. 
As seen in Figure~\ref{fig:misinformation-reddit-user}, as on Twitter, misinformation subReddits as well as have higher levels of toxicity compared with subReddis with not misinformatino submissions. 

Looking a







==> submissions.tex <==
\section{RQ1: Reddit Misinformation Submissions vs Authentic News Submissions}\label{sec:rq1}
Having outlined our methodology, in this section we turn to understand the relative levels of toxicity and polarization orientations of users and subreddits that interact with misinformation and authentic news. 




%\subsection{Misinformation vs Mainstream Submissions}


\subsection{Experimental Setup}
As previously mentioned, on Reddit, users can submit news articles from different websites as a submission under which users can comment and discuss the article or issues prompted by the news article headline. To understand the relative presence of political incivility and toxic comments compelled by misinformation, we thus first compare levels of toxic comments posted under misinformation and authentic news URL submissions.

To do this, across all our collected subreddits we gather the sets the URL submissions that utilize our set of misinformation and authentic news websites. Altogether, within our Pushshift dataset, there were 38,264 different submissions utilizing our first set of 541 misinformation websites from 2,217 different subreddits and 226,930 submissions utilizing our first set of 565 authentic news websites from 18,383 unique subreddits. This difference in magnitude of submissions, we believe, is largely due to the greater popularity and widespread appeal of authentic mainstream news compared with alternative and more fringe websites. Indeed, utilizing the Amazon Alexa Top Million list from March 1, 2021~\cite{amazon-top-mil}, we find that 255 authentic news websites were in the top 100K websites, while only 101 misinformation websites were in the top 100K. To further bolster and confirm our results, we test our findings in this section utilizing our second set of misinformation and mainstream websites. Altogether, from this second set of URLs, we find an additional set of 9,558 misinformation and 560,673 authentic news submissions.

\subsection{Differences in Toxicity/Incivility between Misinformation and Authentic News Submissions}\label{sec:toxicity}

Looking at the toxicity comments from our first set of misinformation domains, we see that 14.9\% of the submission had at least one toxic comment and 1.35\% of all the comments were toxic. In contrast, for the first set of authentic submissions 13.6\% of the submissions had a toxic comment and only 0.85\% of the comments were toxic. We thus see a 60\% uptick in the rate at which toxic comments are posted on the misinformation submissions. Confirming this finding with our second set of 9,558 misinformation and 560,673 authentic news submissions, we again see a similar pattern of higher toxicity in the misinformation submission comments. 15.3\% of the misinformation submissions had toxic comments with 0.92\% of the comments being toxic. In contrast, 11.74\% of the mainstream submissions had toxic comments with 0.64\% of the comments being toxic. We thus see in this replicated experiment that Reddit misinformation conversations indeed have a higher incidence and occurrence of toxicity and incivility. Putting all these conversations together, we find that 1.17\% of comments under misinformation submissions are toxic/uncivil while 0.7\% of comments for authentic news websites are toxic/uncivil. we thus find an overall 63\% increase in the rate at which toxic comments are posted on misinformation submissions.

\begin{figure*}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/user_toxicity_above10.png}
  \caption{URL Set 1}
\label{fig:harmonic-sub1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/user_toxicity_above10_2.png}
    \caption{URL Set 2}
  \label{fig:pagerank-sub2}
\end{subfigure}

\caption{\textbf{Toxicity levels for users who comment under authentic News and misinformation URL Reddit submissions}---Users who interact with misinformation submissions are slightly more toxic/uncivil than users that interact with authentic news. Both groups are slightly more toxic/uncivil than Reddit users generally. }
\label{fig:users-misinformation-authentic-toxicity}
\end{figure*}
%\paragraph{User and Subreddit Toxicity in Misinformation and Mainstream Reddit Submissions }
%  We now seek to eke out some of the causes the higher amount of toxicity within the misinformation URL submissions on Reddit. 


Higher toxicity within misinformation submissions could be caused by (1) more toxic/uncivil users participating in these conversations or (2) higher toxicity norms in the subreddits where the misinformation was posted. As seen in Figure~\ref{fig:users-misinformation-authentic-toxicity}, we see that these users are slightly more toxic than their authentic news counterparts. For the first group of URL submissions, on average 1.54\% of the comments for the users associated with these submissions are toxic/uncivil compared with 1.22\% for the corresponding group of authentic news users. Similarly, on average 1.48\% of comments posted by the second group of misinformation users are toxic compared to 1.32\% for the authentic news commenters. However, for bot URL groups, as seen in Figure~\ref{fig:users-misinformation-authentic-toxicity}, the distributions of their Perspective API scores are fairly close. We note, that despite this proximity in toxicity of misinformation commenters between authentic news commenters, the higher user toxicity appears stable even among users from the same subreddits. Comparing the users who posted in subreddits where \emph{both} mainstream and misinformation URLs were posted, we still see that the users who posted on misinformation submissions had elevated rates of toxicity (1.21\% compared to 1.45\%). We thus see ``more toxic'' users are indeed commenting more on misinformation submissions compared to authentic news submissions. Finally, to further confirm our results, we perform U-Mann Whitney tests to ensure that there are indeed statistically significant differences between the rate of toxicity in misinformation and authentic news users; running these tests finding p-values $<10^{-12}$, we indeed conclude that both groups URL submission commenters that there are indeed higher rates of toxicity for the misinformation users.

However, despite the finding that more toxic users are indeed commenting more often on misinformation submissions, their higher rate of toxicity is not enough to explain the larger amount of toxic comments in misinformation submissions. After accounting for the higher rate of user toxicity across all the URL submissions, we still see 25.4\% more toxic comments than would be expected for the first set of URLs and 28.0\% for the second comparison set. Other factors, besides the specific users that comment on misinformation, are contributing to the higher rate of toxicity on misinformation submissions.



\begin{figure*}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/subreddit_toxicity_above10.png}
      \caption{URL Set 1}
\label{fig:harmonic-sub1}
\end{subfigure}%s
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/subreddit_toxicity_above10_2.png}
      \caption{URL Set 2}
  \label{fig:pagerank-sub2}
\end{subfigure}

\caption{\textbf{Toxicity Levels in Subreddits with Authentic News and Misinformation URL Submission}---Subreddits with misinformation submissions are overall more toxic/uncivil compared with authentic news subreddits and subreddits more generally.}
\label{fig:subreddit-misinformation-authentic-toxicity}
\end{figure*}

Looking at the role of subreddits in promoting toxicity in Figure~\ref{fig:subreddit-misinformation-authentic-toxicity}, we find that the toxicity norms of subreddits with misinformation submissions also contribute to higher levels of toxic comments. We see that on average for both sets of URLs that we consider, the set of subreddits with misinformation submissions have higher levels of toxicity compared to subreddits with authentic news submissions. Altogether, in our first set of misinformation URLs, for corresponding subreddits 1.40\% of comments posted there are toxic/uncivil. This is compared to a corresponding rate of 0.80\% for comments within subreddits with authentic news submissions. We see a similar difference from our second set of URLs (1.1\% vs 0.7\%). From these two datasets, we thus find that users in subreddits with misinformation submissions post toxic comments at a rate between 57\% (second set of URLs) and 75\% (first set of URLs) higher than in subreddits with authentic news submissions. We again perform U-Mann Whitney tests to ensure that there are indeed statistically significant differences between the rate of toxicity in misinformation and authentic news subreddits. With p-values $<10^{-12}$, we conclude that for both groups that there are indeed higher levels of toxicity in the misinformation subreddits.

\subsection{Differences in Political Polarization between Misinformation and Authentic News Submissions}\label{sec:polarization}
Having seen the higher levels of toxicity/incivility present within misinformation Reddit submissions, we now explore the differences in political polarization between users who comment on misinformation and those that comment on authentic news.

\begin{figure*}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/user_political_comparison.png}
      \caption{URL Set 1}
\label{fig:political-users1}
\end{subfigure}%s
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/user_political_comparison2.png}
      \caption{URL Set 2}
  \label{fig:political-users2}
\end{subfigure}

\caption{\textbf{Political polarization of users who comment under authentic news and misinformation Reddit submissions}-- There are not significant differences in political ideology between users who comment on misinformation and those that comment on authentic news. }
\label{fig:users-political-orientation}
\end{figure*}
\begin{figure*}
\begin{subfigure}{.4\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/subreddit_political_comparison.png}
    \caption{URL Set 1}
\label{fig:harmonic-sub1}
\end{subfigure}%s
\begin{subfigure}{.4\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/subreddit_political_comparison2.png}
    \caption{URL Set 2}
  \label{fig:pagerank-sub2}
\end{subfigure}

\caption{\textbf{Political polarization of subreddits with authentic news and misinformation Reddit submissions}--- There are no significant differences in the political orientation of subreddits where misinformation and authentic news appear. }
\label{fig:subreddit-misinformation-authentic-toxicity}
\end{figure*}
Looking at the set of users commenting under misinformation Reddit submissions, we surprisingly do not see dramatic differences between these users and those that comment on authentic news submissions. In fact, as seen in Figure~\ref{fig:users-political-orientation} for both our set of misinformation URL sets, we see a slight leftward tilt in the average commenter. Similarly and surprisingly, looking in Figure~\ref{fig:subreddit-misinformation-authentic-toxicity} at the political orientation of the subreddits where our misinformation submissions appeared, we again see that there is not much difference in their respective polarizations. This appears to indicate that \emph{both} misinformation and authentic news appear within subreddits and get commented on by users across the political spectrum.

%This indicates that the particular higher levels of toxicity observed in our set of misinformation-filled subreddits is not being driven by the political environment of the subreddit. 

We note that despite misinformation appearing in subreddits across the political spectrum, the users that post misinformation have a rightward tilt compared to the users that comment on misinformation. As seen in Figure~\ref{figure:misinformation-posters-commenters}, for both sets of URLs submissions with comments, we see that misinformation submitters are on the whole more conservative than their corresponding more liberal commenters. This is largely in contrast to authentic news commenters and posters. As seen in Figure~\ref{figure:news-posters-commenters}, authentic news posters and commenters share nearly the exact same distribution. 




\begin{figure}
\centering
\begin{subfigure}{.4\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/misinformation_posters_commenters.png}
    \caption{URL Set 1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/misinformation_posters_commenters2.png}
    \caption{URL Set 2}
\end{subfigure}
\caption{\textbf{Distribution of political orientation of posters and commenters of misinformation}--- There is a noticeable rightward tilt in users that post misinformation compared to those that comment on misinformation.}
\label{figure:misinformation-posters-commenters}

\end{figure}



\begin{figure}
\centering
\begin{subfigure}{.4\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/news_posters_comenters_comparison.png}
    \caption{URL Set 1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
\includegraphics[width=1\linewidth]{figures/news_posters_comenters_comparison2.png}
    \caption{URL Set 2}
\end{subfigure}
\caption{\textbf{Distribution of political orientation of posters and commenters of authentic news}--- Unlike for misinformation posts, the posters and the commenters on authentic news share similar distributions of political orientations.}
\label{figure:news-posters-commenters}
\end{figure}

Altogether, we thus observe (especially in contrast to authentic news submissions), that a politically different set of users post misinformation news compared to those that comment on it. While we did not observe that the polarization levels of users who comment on misinformation are substantially different from commenters on authentic users, we did observe that they \emph{are} different from posters of misinformation content. 

\subsection{Intersection of Misinformation, News Media, Toxicity, and Political Polarization across Subreddits}
Finally, having seen the distribution of the political polarization and toxicity among different users and in different environments, we now look if these different characteristics correlate with the amount of misinformation and authentic news in each subreddit. Namely, we seek to determine more broadly if levels of misinformation are correlated with increased levels of toxicity. To do this we rely on our list of \textit{misinfo-oriented} and \textit{mainstream-oriented} websites.



Specifically, for each subreddit in our dataset, we compute their \textit{misinformation similarity} and their \textit{mainstream similarity} based on the percentage of each subreddit's  URL submissions that come from websites that are \textit{misinfo-oriented} and \textit{mainstream-oriented}. This measurement essentially determines the rough approximate percentage of submissions within each of our subreddits that are misinformation oriented/related and the percentage that are mainstream oriented/related. 

\begin{figure}
\begin{minipage}[l]{0.6\textwidth}
\includegraphics[width=1\columnwidth]{figures/cross_graphs.png} 
\end{minipage}
\begin{minipage}[l]{0.35\textwidth}
\caption{\textbf{Misinformation, toxicity, and political polarization interactions}--- As subreddits increase in misinformation levels, they become more toxic. However, there is not a large correlation between misinformation levels and the political polarization of subreddits. Similarly, we do not see any correlation between political polarization levels and mainstream similarity; nor do we see any correlation with toxicity levels.\label{figure:cross-graph} }
\end{minipage}

\end{figure}


As seen in Figure~\ref{figure:cross-graph}, across all our 46K considered subreddits, we observe that as subreddits become more similar to misinformation and hyperlink to more \textit{misinfo-oriented} domains, their toxicity increases. This largely matches our observation in Section~\ref{sec:toxicity} that misinformation submissions are in general more toxic/uncivil than authentic news submissions. Misinformation levels in general thus appear to be correlated with increased toxicity. We further again surprisingly see in Figure~\ref{figure:cross-graph} that levels of misinformation are not heavily correlated with political polarization. It does not appear that the most politically polarized environments necessarily rely upon misinformation. For example, the most left-leaning subreddits (Table~\ref{table:mostpolitical-subreddits}) that we observed mostly supported US Senator Bernie Sanders and did not necessarily have high misinformation levels. Conversely, we do not see much of a correlation between subreddits with high mainstream similarity and political polarization and toxicity. This again reinforces our results finding that mainstream news does not have higher levels of toxicity and political polarization level from Section~\ref{sec:toxicity} and Section~\ref{sec:polarization}. We thus see again from this analysis that misinformation is indeed correlated with higher toxicity, while authentic news is largely not. 
%\subsection{Reddit Level Interactions}
%Before examining the interaction directly within


\subsection{Summary}
In this section, we found that misinformation on Reddit largely is correlative with and predictive of higher amounts of incivility and toxicity on the platform. Most markedly, we observed that the comments under misinformation submissions are posted at a rate 60\% higher than the comments under authentic news submissions. Further, while we do observe a dichotomy in the political polarization of users that post misinformation and those that comment on misinformation, somewhat surprisingly, we find that misinformation appears across different political environments, with it not being concentrated just in the political extremes. Lastly, looking at how different levels of misinformation correlate with toxicity, we find the more \textit{misinfo-oriented} submissions a given subreddit has, the more toxic/uncivil it is likely to be. 

 

==> twitter.tex <==
\section{Borderless: Twitter Misinformation and Political Communities}
In this section, we analyze the interplay between the penchant towards political polarization, toxicity, and misinformation on social media users. Previous works have indicated that toxicity levels are heavily tied with users' political polarization levels~\cite{chipidza2021effect,kim2021distorting} as well as their penchant to conspiratorial content~\cite{hanley2021no}. We now investigate how toxic and political polarized communities contribute to the propagation of misinformation and conspiracies by individuals users on Twitter.  

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/LevelsOfMisinformationAndNewsOnTwitter.png} 
\caption{\textbf{Number of Authentic News, Misinformation, and Conspiracy Theory Links on Twitter in 2020}--- Misinformation maintains a large presence of Twitter, with about half as many links as authentic news. Conspiracy websites having a relatively small but non-negligible presence on the platform. 
}
\label{figure:levels_of_misinfo}
\end{figure}

As seen in Figure~\ref{figure:levels_of_misinfo}, counting the number of instances of misinformation, authentic news, and conspiracy theory hyperlinks based on a 1\% Twitter sampling over 6 months, there are consistent levels of misinformation news articles tweeted. The amount of misinformation links from users, in fact largely follows the amount of authentic news tweeted. Specifically, we find a Pearson correlation of 0.711 between the number of misinformation URLs posted and the number of authentic news posted.  At any given time, the amount of misinformation links within our dataset varies from, $\frac{1}{3}$ to $\frac{1}{2}$ of the amount of authentic news hyperlinks posted. Comparing this to a set of non-news related URLS as well as a set of random domains (chosen randomly from the Amazon Alexa Top 1M from January 1 2022), we see that the changing amounts of misinformation and news based URLs in our dataset is largely due to the vicissitudes of the news cycles rather than as an artifact of our dataset. 

Having established the relative levels of misinformation on Twitter, we now seek to understand some of the drivers behind misinformation heavy Twitter accounts. Taking all URLS within our dataset, we acquire 189K different Twitter accounts that tweets authentic news, misinformation, or conspiracy theories during the month of January. Within this set of Twitter accounts 139663 accounts tweeted at least one authentic news website and 115073 accounts tweeted at least one misinformation website. Using the Tweepy API, we collect the last 3240 tweets of each of these users, giving us a dataset of 446,439,819 tweets total. 

\begin{figure*}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/all-correlations.png}
  \caption{All User Correlations}
\label{fig:twitter-reddit-partisanship-time}
\end{subfigure}%
\hspace{20pt}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/republican-correlations.png}
  \caption{Republican User Correlations}
  \label{fig:twitter-reddit-partisanship}
\end{subfigure}
\hspace{20pt}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/democratic-correlations.png}
  \caption{Democratic User Correlations}
  \label{fig:twitter-reddit-toxicity-time}
\end{subfigure}
\caption{\textbf{Twitter User Characteristic Correlations}--- Among different 
}
\label{fig:twitter-correlations}
\end{figure*}

After labeling each tweet with the Perspective API and gathering each accounts approximate partisanship, partisanship URL variance, and misinformation promotion levels, we now seek to understand the factors behind accounts promoting misinformation. As a proxy for the misinformation promotion level of given Twitter users, we utilize the percentage of the URLs that they post that belong to our set of misinformation domains.

As seen in Figure~\ref{fig:twitter-correlations}, there is a high degree of correlation between the political polarization of users and misinformation levels of users. This largely concurs with prior research that suggests that political polarization is the most potent reason behind the sharing of ``fake-news'' on Twitter~\cite{osmundsen2021partisan}. Looking at users whose average URL posted is conservative/Republican, this is especially prominent,  with polarization having a 0.70 Pearson correlation with levels of misinformation on their accounts. 


We also see, somewhat counter-intuitively, at a given level of partisanship, as the partisanship variance of individuals accounts increases, the amount of misinformation that that account post also increases. This suggests that users that actually engage with materials/hyperlink to materials that are substantially different from the average political information that they hyperlink to are more likely to post misinformation. Bucking our initial expectations, engaging with more and different sources is associated with heavier amounts of misinformation. Prior work~\cite{starbird2018ecosystem} has noted the political echo chambers that promote misinformation online. However, this appears to be only a part of the story of the spread of misinformation. 
\begin{comment}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/misinformation-graph-partisan-var.png} 
\caption{\textbf{Partisanship and Partisanship Variance Affect on Misinformation}--- As users become more politically hardened and engage with a higher amount of news sources, they are more likely to post misinformation. While not exact, as levels of variety of political URLS posted increases at each level of partisanship, the the levels of misinformation increases as well. This is seen by the red fraying at the edges of the graph.  
}
\label{figure:partisanship-misinfo-variance}
\end{figure}
\end{comment}
As seen in Figure~\ref{figure:partisanship-misinfo-variance}, it is the set of users that have the highest variance of political URLs as well as the most highly partisan users that have the highest levels of misinformation on their Twitter accounts.For example one particularly highly misinformation-dense account (Figure~\ref{fig:twitter-misinformation2}) linked to a video from MSNBC to deride one of its hosts. This is not to say that these users regularly link to highly opposing views often; however, this tendency to interact with substantially different than a user's political average results in a higher likelihood of misinformation. 
\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/liberal-graph-partisan-misinformation.png}
\label{fig:left-twitter-pol-toxicity}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/conservative-graph-partisan-misinformation.png}
  \label{fig:right-twitter-pol-toxicity}
\end{subfigure}
\caption{\textbf{Average Misinformation Levels as a function of average political bias and tendency to post opposing views}-- Users that post the URLs of websites that are against their average political bias are more likely to post misinformation.
}
\label{fig:twitter-pol-toxicity}
\end{figure*}

Users that post more URLs that are opposed to their mean political URLs/belief also show a higher probability of toxicity compared to other users of similar political averages. Plotting levels of toxicity as a function of political bias and the tendency to post opposing views (URLs from websites that are conservative-leaning for Democratic voters and vice versa), we see 1) that levels of toxicity are highly connected with levels of partisanship ( Pearson correlation of 0.38 for all users), and 2) that as the number of URLs from websites with opposing views increases, we see that average levels of toxicity increase as well. Looking at Figure \ref{fig:twitter-pol-toxicity} and , we  that for both left-wing and right-wing users, similarity at each given partisanship level, as the percentage of URLs from websites that oppose their mean political bias increases, that mean levels of toxicity increases with users at the end of each level of partisanship showing the highest levels of toxicity. For liberal leaning users, we find that after normalizing for partisanship, a Pearson correlation of 0.242 between the average toxicity of a user and their tendency to post URLs opposing their political bias. Just looking at decidedly conservative users with an average political bias of 0.1 or greater, this correlation increases to 0.302. For conservative users, we find that after normalizing for partisanship, the tendency to post opposing views accounts, has a Pearson correlation of 0.240 with their average toxicity. Just looking at decidedly conservative users with an average political bias of 0.1 or greater, this correlation increases to 0.302. As seen, users with the tendency to post URLS against their political bias have higher associated levels of toxicity. This largely mirrors  the tendency to also post misinformation as previously discussed. 

\begin{figure*}
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/high-var-user-tweet1.png}
\label{fig:twitter-misinformation1}
\end{subfigure}%
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/high-var-user-tweet2.png}
  \label{fig:twitter-misinformation2}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/high-var-user-tweet3.png}
  \label{fig:twitter-misinformation3}
\end{subfigure}
\caption{\textbf{Examples of partisan users engaging with material from across the political aisle }-- Highly partisan and misinformation dense Twitter accounts occasional respond to and engage with news stories from authentic news. As pictured, users often deride these sources or cite that stories are  highly divisive.
}
\label{fig:twitter-misinformation-levels}
\end{figure*}

%% Likelihood to post a right-leaning URL if left wing vs probability to post a left-wing URL if right leaning as a function of partisanship 
\begin{figure*}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/republican-democratic-graph.png}
  \caption{Partisanship Levels}
\label{fig:twitter-average-partisanship}
\end{subfigure}%
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/partisan-variance-graph.png}
  \caption{Partisanship Variance}
  \label{fig:twitter-variance-partisanship}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/toxicity-graph.png}
  \caption{Perspective Toxicity }
  \label{fig:twitter-toxicity}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/misinformation-graph.png}
  \caption{Misinformation }
  \label{fig:twitter-misinformation}
\end{subfigure}
\vspace{5pt}
\caption{\textbf{Interconnections between Twitter users with corresponding levels of partisanship, levels of sharing differently partisan sourced articles, toxicity, and levels of misinformation }-- As seen in the above graphs, highly conservative/Republican users and highly democratic/Republican users largely reference each other. Among these highly polarized communities, these users share more disparate and polarized articles, spread more misinformation, and are more toxic.
}
\label{fig:graph-correlations}
\end{figure*}

The tendency of user with higher levels of toxicity, higher levels of partisanship, and higher likelihoods to post misinformation further carries over to Twitter communities that many of these users participate in. Looking at the set of Twitter users in our scrape that posted at leas 300 URL (top 30K users in our dataset), we see this distinction visually. We plot Twitter mention graphs with edge weights based on how often each user mentions other users in their Tweets. Based on how often each user mentions another and clustering the graph using the Force Atlas 2 algorithm, we see two distinctive clusters of conservative/Republican and liberal/Democratic users form. As seen in Figure~\ref{fig:twitter-average-partisanship}, highly partisan users largely group and interact together, with conservative users mentioning other conservative users more frequently and vice versa. Looking a homophily (the tendency of users to mention/reference users of similar political bias as themselves) we see a moderately high value of 0.604. Comparing the graphs, in


As seen in Figure~\ref{fig:graph-correlations}, the cluster of highly liberal/Democratic and highly conservative/Republican users (Figure ~\ref{fig:twitter-average-partisanship}) corresponds to the set of users with higher amounts of political variance in the URLs that they tweet (Figure ~\ref{fig:twitter-variance-partisanship}) as well as the higher amounts of misinformation (Figure ~\ref{fig:twitter-misinformation}).

Looking at the graph of partisanship variance and the the graph of partisanship levels in Figure~\ref{fig:graph-correlations}, and the corresponding levels of correlation in between partisanship and partisanship variance, the most highly partisan accounts are the ones that hyperlink to a variety of different sources. This is particular true of Republican/conservative users. This can be most clearly seen in the dark pink cluster of the partisanship variance graph corresponding heavily with the Conservative/Republican red of the partisanship levels cluster, and finally dark orange cluster of the misinformation graph. 

